Musical Score Following and Audio Alignment

Real-time tracking of the position of a musical performance on a musical score, i.e. score following, can be useful in music practice, performance and production. Example applications of such technology include computer-aided accompaniment and automatic page turning. Score following is a challenging task, especially when considering deviations in performance data from the score stemming from mistakes or expressive choices. In this project, the extensive research present in the field is first explored before two open-source evaluation testbenches for score following--one quantitative and the other qualitative--are introduced. A new way of obtaining quantitative testbench data is proposed, and the QualScofo dataset for qualitative benchmarking is introduced. Subsequently, three different score followers, each of a different class, are implemented. First, a beat-based follower for an interactive conductor application--the TuneApp Conductor--is created to demonstrate an entertaining application of score following. Then, an Approximate String Matching (ASM) non-real-time follower is implemented to complement the quantitative testbench and provide more technical background details of score following. Finally, a Constant Q-Transform (CQT) Dynamic Time Warping (DTW) score follower robust against major challenges in score following (such as polyphonic music and performance deviations) is outlined and implemented; it is shown that this CQT-based approach consistently and significantly outperforms a commonly used FFT-based approach in extracting audio features for score following.

==> 02_parts/02_testbench/chapters/04_discussion.tex <==
\chapter{Discussion}
\label{tb_discussion}
\epigraph{\itshape Music is very abstract. When we talk about music, we're not discussing the music itself but rather how we react to it.}{Daniel Barenboim}

